JPEG Inspired Deep Learning

Although it is traditionally believed that lossy image compression, such as JPEG compression, has a negative impact on the performance of deep neural networks (DNNs), it is shown by recent works that well-crafted JPEG compression can actually improve the performance of deep learning (DL). Inspired by this, we propose JPEG-DL, a novel DL framework that prepends any underlying DNN architecture with a trainable JPEG compression layer. To make the quantization operation in JPEG compression trainable, a new differentiable soft quantizer is employed at the JPEG layer, and then the quantization operation and underlying DNN are jointly trained. Extensive experiments show that in comparison with the standard DL, JPEG-DL delivers significant accuracy improvements across various datasets and model architectures while enhancing robustness against adversarial attacks. Particularly, on some fine-grained image classification datasets, JPEG-DL can increase prediction accuracy by as much as 20.9%. Our code is available on https://github.com/AhmedHussKhalifa/JPEG-Inspired-DL.git.

==> Sections/Methodology_bkp.tex <==
\section{JPEG-DL: JPEG Inspired DL}

\subsection{Problem Formulation}

Given a DNN, let $\mathcal{L}$ denote the loss function used during the training stage, and let $f_{\theta}(.)$ represent the DNN model with trainable weights $\theta$. Consider a pair of random variables $(X, Y)$, where $X \in \mathcal{X}$ represents a raw input image, and $Y$ is the corresponding ground truth label. The distribution of $(X, Y)$ defines the underlying training set. In the standard DL, the primary objective is to solve the following minimization problem:
\begin{equation}\label{eq:general}
\min_{\theta }~\mathbb{E}_{(X,Y)} \mathcal{L} \left( f_{\theta}(X), Y \right).  
\end{equation}

In the JPEG pipeline, as described by \cite{wallace1992jpeg}, the forward process starts by converting the image $x$ from RGB to the YCbCr color and then it is partitioned into $B$ non-overlapping $8 \times 8$ blocks where DCT is applied to each of these non-overlapping blocks to obtain DCT coefficients. Hereafter, the DCT coefficients, denoted as $z$, are then flattened in each block using a zigzag order, arranging $M=$ 64 frequency components, with the first being the DC component and the rest being AC components, ordered from low to high frequencies. All preceding operations are differentiable; however, we did not consider training them in our framework.


In the resulting set of the DCT coefficient sequences $\{z_m\}^{M}_{m=1}$, each sequence $z_m = \{z_{m,n}\}^B_{n=1}$ of length $B$ corresponds to a distinct DCT frequency position, where ${1 \leq m \leq M}$. These different frequency sequences can be modelled as independent sources. Without loss of generality, each DCT source $z_i$ is assumed to have zero mean, otherwise, the mean should be subtracted. For DCT coefficient quantization, we define a quantization table $Q = \{q_1, q_2, \dots, q_M\}$, where $q_m$ is the quantization step size for $z_m$. Each of the luminance and chrominance channel will have a quantization table, respectively. In the standard uniform quantizer, referred as $Q_u$ and also known as hard quantization, DCT coefficients $z_{m,n}$ are quantized to the closest DCT indices $i_{m,n} = \round{z_{m,n}/q_m}$ using the rounding operation, and then reconstructed with $Q$ following $\hat{z}_{m,n} = i_{m,n} \times q_m$, where $\hat{z}$ represents the reconstructed DCT coefficients. For notational simplicity, we will denote all preceding operations with $\mathcal{J}(.;\phi)$ parameterized with $\phi$, where  $\phi$ represents any operation within the pipeline to be designed. However, the key challenge is the non-differentiability of the rounding operation with respect to the input image $x$, which limits the $Q$ from being jointly trained with the underlying DNN model $f_{\theta}$ in a standard DL training pipeline. Our primary goal in the sequel sections is to address this limitation and highlight the key differences between our framework and previous approaches that utilized JPEG to improve DNN performance, as discussed in Section \ref{sec:backgorund}. 

We can reinterpret the conventional formulation in (\ref{eq:general}) to incorporate the method proposed by \cite{yang2021compression}. The authors introduced a new DNN topology that can be represented as $f_{\theta}(.)$, where they are optimizing over its weight $\theta$. In this context, $\phi$ in $\mathcal{J}(.;\phi)$ represents a deterministic compression strategy used to generate compressed samples as inputs for each branch in this topology, as formulated in (\ref{eq:compression_helps}). In contrast, the methods proposed by \cite{salamah2024jpeg} and \cite{JPEG_Compliant} involve a fixed pre-trained model $f_{\theta}(.)$ where the optimization is performed over the compression algorithm $\phi$ in $\mathcal{J}(.;\phi)$, constrained by a target rate, as formulated in (\ref{eq:opts}). The primary limitation of prior work is the inability to jointly optimize both the model weights $\theta$ and the compression algorithm $\phi$, as demonstrated in our joint optimization framework in (\ref{eq:general_jpeg}).

\begin{align}\label{eq:compression_helps}
\min_{\theta }& ~~\mathbb{E}_{(X,Y)} \mathcal{L} \left( f_{\theta}(\mathcal{J}(X;\phi)), Y \right).  
\end{align}

\begin{align}\label{eq:opts}
\min_{\phi }& ~~\mathbb{E}_{(X,Y)} \mathcal{L} \left( f_{\theta}(\mathcal{J}(X;\phi)), Y \right) & \textbf{s.t.} & ~~ R(\phi) \leq R_{T} 
\end{align}

\begin{equation}\label{eq:general_jpeg}
\min_{(\theta, ~\phi) }~\mathbb{E}_{(X,Y)} \mathcal{L} \left( f_{\theta}(\mathcal{J}(X;\phi)), Y \right).  
\end{equation}



\subsection{Differentiable Soft Quantizer}

This soft quantizer is derived based on a probabilistic quantizer, introduced by \cite{yang_patent}, which uses a trainable conditional probability mass function parameterized by a quantization step $q_i$ and a scaling factor $\alpha_i$ that are shared across all blocks $B$ for each frequency $z_i$. Each probabilistic quantizer has a corresponding soft deterministic counterpart, dubbed as \textit{Differentiable Soft Quantizer} ($Q_d$), which is the conditional expectation of the probabilistic quantizer. 



To define the probabilistic quantizer ${Q_p(\cdot)}$, we first need to construct the conditional probability mass function (CPMF) ${P_\alpha(\cdot|z)}$. Let's denote the index set of a uniform quantization as follows:  
\begin{align}
\mathcal{A}&= \{ -L, -L+1, -L+2, \dots, 0, \dots, L-1, L \}.   
\end{align}
For convenience, $\mathcal{A}$ is also regarded as a vector of dimension $2L+1$. Multiplying $\mathcal{A}$ by a quantization step-size $q$, we get the corresponding reconstruction space
 \begin{align}
  \hat{\mathcal{A}} = q \times [-L, -L+1, -L+2, \dots, 0, \dots , L-1, L].    
\end{align}
Again, we will regard $ \hat{\mathcal{A}} $ as both a vector and set. 


The DCT coefficient located at frequency $i$ and block $j$ is represented by ${z_{i, j}}$, where ${1 \leq i \leq M}$ and ${1 \leq j \leq B}$. $z$ is randomly quantized to ${\hat{z} \in  \hat{\mathcal{A}}}$. A trainable CPMF $ {P_{\alpha}(\cdot | z) }$ is defined below over the reproduction alphabet $ \hat{\mathcal{A}}  $ or equivalently the index set $\mathcal{A}$ given $z$, where ${\alpha >0 }$ can be a hyper parameter or a trainable parameter: 
 \begin{equation} \label{eq:CPMF}
     P_{\alpha}(\hat{z} | z) = \frac{e^{-\alpha (z - \hat{z})^2}}{\sum_{j \in \mathcal{A}} e^{-\alpha (z - jq)^2 }}, ~\forall \hat{z} = i q, ~i \in \mathcal{A}.
 \end{equation}
Expand $z$ to dimension ${2L+1}$
\begin{align}
\big[z \big]_{2L+1} =   [\underbrace{z, \dots, z}_{\text{$2L+1$ times}}].
\end{align}
 The CPMF ${ P_{\alpha}(\cdot | z) }$ can be easily computed via the softmax operation and viewed as a vector of dimension ${2L+1}$. 
\begin{align} \label{eq:PMF}
 \big[P_{\alpha}(\cdot | z) \big]_{2L+1} &= \boldsymbol{\sigma} \Big(- \alpha \times \left(  \big[ z \big]_{2L+1} -   \hat{\mathcal{A}} \right)^2 \Big),
\end{align}
where ${\boldsymbol{\sigma}(\cdot)}$ denotes the softmax operation. 

With the CPMF ${ P_{\alpha}(\cdot | z)  }$,  $z$ is now quantized to each  ${\hat{z} \in \hat{\mathcal{A}} }$ with probability ${P_{\alpha}(\hat{z} | z)}$. Denote this random mapping by 
\begin{align} \label{eq:Qprob}
\hat{z} =  {Q}_{\rm p}(z).   
\end{align}
Note that given $z$, ${\hat{z}}$ is a random variable taking values in ${\hat{\mathcal{A}}}$ with distribution ${ P_{\alpha}(\cdot | z)}$. However, as $\alpha$ approached infinity, $Q_p(z)$ will quantize $z$ to the nearest point in  $\hat{\mathcal{A}}$, effectively functioning as a uniform quantizer, also known as a hard decision quantizer. 


When the probabilistic quantizer $Q_p(z)$ is used into the DL training pipeline, how can the gradients with respect to (w.r.t.) $z$, $q$ and $\alpha$ be computed during backward passes for joint training with the underlying model $f_{\theta}(.)$? 

Given $z$, instead of the random mapping ${{Q}_{\rm p}}(.)$, a soft deterministic version ${{Q}_{d}(\cdot)}$ is defined based on the conditional expectation of ${\hat{z}=iq}$ given $z$, i.e., 
\begin{align} \label{eq:softQ}
{Q}_{\rm d}(z) = \mathbb{E} \{\hat{z} |z \}  = \sum_{i \in {\mathcal{A}}} P_{\alpha}(iq|z) ~iq.    
\end{align}

For those familiar with the self-attention mechanism proposed by \citet{vaswani2017attention}, $Q_d(.)$ can be viewed as analogous to Scaled Dot-Product Attention, as discussed in Appendix (\ref{app:Scaled_Dot-Product}).

Given the relationship between $Q_d$ and $Q_p$ in (\ref{eq:softQ}), the proposed formulation in (\ref{eq:general_jpeg}) can be resolved. 
By considering $\phi$ in $\mathcal{J}(x;\phi)$ to be represented by $Q_d$ within our JPEG-DL framework, we enable joint optimization with the underlying model. However, it is crucial to show that $Q_d$ can effectively approximate $Q_p$, providing an analytic formula for calculating partial derivatives with respect to $z$, $q$ and $\alpha$. This is discussed in the following subsection.


\subsection{Training DNN Jointly with JPEG Compression}
Given $z$, the expected distortion (defined as the squared error) between $z$ and ${{Q}_{\rm p}(z)}$ given $z$ can be expressed as below.

\begin{align} \label{eq:expdistortion}
\mathbb{E} \{(z-Q_{\rm p}(z))^2 |z \} = (z-Q_{\rm d}(z))^2 + Var\{Q_{\rm p}(z) | z\}.
\end{align}

where ${Var\{Q_{\rm p}(z) | z\}}$ is the conditional variance of ${Q_{\rm p}(z)}$ given $z$. ${Var\{Q_{\rm p}(z) | z\}}$ is negligible when $\alpha$ is sufficiently large. Therefore ${{Q}_{\rm d}(z)}$ can be used to approximate the probabilistic quantizer ${Q_{\rm p}(z)}$. Consequently, the soft differentiable variant of the probabilistic quantizer offers an analytic formula for gradient calculation during training with respect to both the raw input $x$ and the quantization parameters $q$ and $\alpha$.  For more details on the analytic formulas, please refer to Appendix (\ref{app:Partial_Derivatives}). 

To illustrate the inner workings of $Q_d(z)$ and how the quantizer softness is affected by changing the values of $q$ and $\alpha$, we present real examples with a realization of the random variable $z$, denoted as $z$, for two different DCT frequencies in Fig. \ref{fig:jpeg_dl_b}. The quantization is considered soft because the output is not restricted strictly in the reproduction space $\hat{\mathcal{A}}$; instead, it preserves a level of continuous representation, allowing for a softer change between quantization levels. As observed, $Q_d$ introduces additional non-linearity, which will help the underlying model to capture intricate feature relationships and non-obvious patterns in the raw input.



==> Sections/fine_grained_table.tex <==
\begin{table}[!ht]
\caption{Top-1 validation accuracy (\%) on various fine-grained image classification tasks and model architectures. We report the mean and standard deviation of experimental results over three runs.}
\vspace{-3mm}
\small
\begin{center}
% luo2020rate
% \def\arraystretch{1.5}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|c|c|c}
\toprule
Dataset & Method & ResNet-18 & DenseNet-121 \\
\midrule
\multirow{10}{*}{CUB-200} & \cellcolor{red!30} Baseline & {{54.00}\ms{1.43}\hfill} \, (-4.81)  & {{57.70}\ms{0.44}\hfill} \, (-3.62) \\ 
\cmidrule{2-4}
& \cellcolor{orange!30} Rand.~QF ~~~~~~~[1:50] & {52.86\ms{0.69}\hfill} \, (-5.95) & {55.72\ms{0.72}\hfill} \, (-5.60)   \\ 
& \cellcolor{orange!30} Rand.~QF~~~~[50:100] & {54.53\ms{0.41}\hfill} \, (-4.28) & {56.98\ms{0.90}\hfill} \, (-4.34)   \\ 
& \cellcolor{orange!30} Rand.~QF ~~~~ [1:100]  & {53.91\ms{0.43}\hfill} \, (-4.90) & {57.20\ms{0.33}\hfill} \, (-4.12)   \\ 
\cmidrule{2-4}
& \cellcolor{yellow!50} Denoising & {54.82\ms{0.40}\hfill} \, (-3.99) & {56.02\ms{1.00}\hfill} \, (-5.30)   \\ 
& \cellcolor{yellow!50} Equalization & {49.00\ms{0.31}\hfill} \, (-9.81) & {54.32\ms{0.57}\hfill} \, (-7.00)   \\ 
\cmidrule{2-4}
& \cellcolor{blue!20} Learnable Resize & {54.98\ms{0.19}\hfill} \, (-3.83) & {57.35\ms{0.22}\hfill} \, (-3.97)   \\ \cmidrule{2-4}
& \cellcolor{green!40}  JPEG-DL (4:2:0)& {58.00\ms{0.12}\hfill} \, (-0.81) & {60.55\ms{0.71}\hfill} \, (-0.77)   \\
& \cellcolor{green!40} JPEG-DL (4:2:2) & {58.11\ms{0.10}\hfill} \, (-0.70) & {\textbf{61.51}\ms{0.41}\hfill} \, (+0.19)   \\
& \cellcolor{green!40} JPEG-DL (4:4:4) & {\textbf{58.81}\ms{0.12}\hfill} \,    & {61.32\ms{0.43}\hfill} \,   \\
\midrule
\multirow{10}{*}{Dogs} &  \cellcolor{red!30} Baseline & {{63.71}\ms{0.32}\hfill} \, (-1.86) & {{66.61}\ms{0.17}\hfill} \,  (-3.06) \\
\cmidrule{2-4}
& \cellcolor{orange!30}  Rand.~QF ~~~~~~~[1:50]& {60.61\ms{0.17}\hfill} \, (-4.96) & {64.93\ms{0.17}\hfill} \, (-4.74)   \\ 
& \cellcolor{orange!30}  Rand.~QF~~~~[50:100] & {63.14\ms{0.30}\hfill} \, (-2.43) & {66.97\ms{0.18}\hfill} \, (-2.70)   \\ 
& \cellcolor{orange!30} Rand.~QF ~~~~ [1:100]   & {62.12\ms{0.16}\hfill} \, (-3.45) & {65.59\ms{0.54}\hfill} \, (-4.08)   \\ 
\cmidrule{2-4}
& \cellcolor{yellow!50} Denoising & {62.52\ms{0.41}\hfill} \, (-3.05) & {66.36\ms{0.34}\hfill} \, (-3.31)   \\ 
& \cellcolor{yellow!50} Equalization & {62.38\ms{0.29}\hfill} \, (-3.19) & {67.12\ms{0.19}\hfill} \, (-2.55)   \\ 
\cmidrule{2-4}
& \cellcolor{blue!20} Learnable Resize & {63.10\ms{0.43}\hfill} \, (-2.47) & {67.90\ms{0.32}\hfill} \, (-1.77)   \\ \cmidrule{2-4}
& \cellcolor{green!40}  JPEG-DL (4:2:0)& {65.57\ms{0.31}\hfill} \, (+0.00) & {68.90\ms{0.08}\hfill} \, (-0.77)   \\
& \cellcolor{green!40} JPEG-DL (4:2:2) & {\textbf{65.64}\ms{0.16}\hfill} \, (+0.07) & {\textbf{69.85}\ms{0.78}\hfill} \, (+0.18)   \\
& \cellcolor{green!40} JPEG-DL (4:4:4) & {65.57\ms{0.37}\hfill} \,  & {69.67\ms{0.58}\hfill} \,   \\
\midrule
\multirow{10}{*}{Flowers} & \cellcolor{red!30} Baseline & {{57.13}\ms{1.28}\hfill} \, (-11.63) & {{51.32}\ms{0.57}\hfill} \,  (-20.90) \\
\cmidrule{2-4}
& \cellcolor{orange!30}  Rand.~QF ~~~~~~~[1:50]& {58.33\ms{0.48}\hfill} \, (-10.43) & {51.44\ms{0.79}\hfill} \, (-20.78)   \\ 
& \cellcolor{orange!30}  Rand.~QF~~~~[50:100] & {55.98\ms{0.89}\hfill} \, (-12.78) & {51.67\ms{1.10}\hfill} \, (-20.55)   \\ 
& \cellcolor{orange!30} Rand.~QF ~~~~ [1:100]   & {57.55\ms{0.66}\hfill} \, (-11.21) & {52.32\ms{0.73}\hfill} \, (-19.90)   \\ 
\cmidrule{2-4}
& \cellcolor{yellow!50} Denoising & {57.28\ms{1.06}\hfill} \, (-11.48) & {50.37\ms{0.79}\hfill} \, (-21.85)   \\ 
& \cellcolor{yellow!50} Equalization & {60.56\ms{0.98}\hfill} \, (-8.20) & {61.72\ms{0.21}\hfill} \, (-10.50)   \\ 
\cmidrule{2-4}
& \cellcolor{blue!20} Learnable Resize & {57.41\ms{0.48}\hfill} \, (-11.35) & {51.21\ms{0.82}\hfill} \, (-21.01)   \\ \cmidrule{2-4}
& \cellcolor{green!40}  JPEG-DL (4:2:0)& {67.58\ms{1.50}\hfill} \, (-1.18) & {68.01\ms{1.17}\hfill} \, (-4.21)   \\
& \cellcolor{green!40} JPEG-DL (4:2:2) & {67.75\ms{1.19}\hfill} \, (-1.01) & {68.79\ms{1.08}\hfill} \, (-3.43)   \\
& \cellcolor{green!40} JPEG-DL (4:4:4) & {\textbf{68.76}\ms{0.57}\hfill} \, & {\textbf{72.22}\ms{1.05}\hfill} \,   \\
\midrule
\multirow{10}{*}{Pets} & \cellcolor{red!30} Baseline & {{70.37}\ms{0.84}\hfill} \, (-4.47) & {{70.26}\ms{0.79}\hfill} \, (-5.64) \\
\cmidrule{2-4}
& \cellcolor{orange!30}  Rand.~QF ~~~~~~~[1:50]& {69.71\ms{0.54}\hfill} \, (-5.13) & {68.93\ms{0.50}\hfill} \, (-6.97)   \\ 
& \cellcolor{orange!30}  Rand.~QF~~~~[50:100] & {70.00\ms{0.57}\hfill} \, (-4.84) & {68.63\ms{0.82}\hfill} \, (-7.27)   \\ 
& \cellcolor{orange!30} Rand.~QF ~~~~ [1:100]   & {69.52\ms{0.62}\hfill} \, (-5.32) & {70.60\ms{1.05}\hfill} \, (-5.30)   \\ 
\cmidrule{2-4}
& \cellcolor{yellow!50} Denoising & {69.15\ms{1.07}\hfill} \, (-5.69) & {69.03\ms{1.13}\hfill} \, (-6.87)   \\ 
& \cellcolor{yellow!50} Equalization & {73.00\ms{0.79}\hfill} \, (-1.84) & {75.04\ms{1.30}\hfill} \, (-0.86)   \\ 
\cmidrule{2-4}
& \cellcolor{blue!20} Learnable Resize & {70.04\ms{0.72}\hfill} \, (-4.80) & {68.83\ms{1.85}\hfill} \, (-7.07)   \\ \cmidrule{2-4}
& \cellcolor{green!40}  JPEG-DL (4:2:0)& {74.64\ms{1.34}\hfill} \, (-0.20) & {\textbf{76.21}\ms{0.35}\hfill}  \, (+0.31)   \\
& \cellcolor{green!40} JPEG-DL (4:2:2) & {74.81\ms{0.51}\hfill} \, (-0.03) & {76.17\ms{1.83}\hfill} \, (+0.27)   \\
& \cellcolor{green!40} JPEG-DL (4:4:4) & {\textbf{74.84}\ms{0.66}\hfill} \,   & {75.90\ms{0.68}\hfill} \,    \\
\bottomrule
\end{tabular}}
\end{center}
\label{table:fine_grained_all}
\end{table}

